Reputation Dynamics in a Market for Illicit Drugs

We analyze reputation dynamics in an online market for illicit drugs using a novel dataset of prices and ratings. The market is a black market, and so contracts cannot be enforced. We study the role that reputation plays in alleviating adverse selection in this market. We document the following stylized facts: (i) There is a positive relationship between the price and the rating of a seller. This effect is increasing in the number of reviews left for a seller. A mature highly-rated seller charges a 20% higher price than a mature low-rated seller. (ii) Sellers with more reviews charge higher prices regardless of rating. (iii) Low-rated sellers are more likely to exit the market and make fewer sales. We show that these stylized facts are explained by a dynamic model of adverse selection, ratings, and exit, in which buyers form rational inferences about the quality of a seller jointly from his rating and number of sales. Sellers who receive low ratings initially charge the same price as highly-rated sellers since early reviews are less informative about quality. Bad sellers exit rather than face lower prices in the future. We provide conditions under which our model admits a unique equilibrium. We estimate the model, and use the result to compute the returns to reputation in the market. We find that the market would have collapsed due to adverse selection in the absence of a rating system.

==> figures/estimates_offline.tex <==
% latex table generated in R 3.3.1 by xtable 1.8-2 package
%
\begin{tabular}{llr}
  \toprule
Parameter & Variable & Estimate \\
  \midrule
Low type value & $\underline{\theta}^\text{offline}$ & 0.354 \\
  High type value & $\overline{\theta}^\text{offline}$ & 0.439 \\
  Fraction of entering high type & $\alpha^\text{offline}$ & 0.263 \\
  Probability of moving up in sales & $\gamma^\text{offline}$ & 0.370 \\
  Standard deviation of rating process & $\sigma_r^\text{offline}$ & 0.199 \\
  Standard deviation of prices & $\sigma_p^\text{offline}$ & 0.129 \\
\end{tabular}


==> section/moralhazard.tex <==
%!TeX root = ../draft.tex

The seller has two possible decision problems to solve. The first decision problem corresponds to the case in which the seller cannot switch qualities. In this case, he only has an exit decision to make, and it is trivial to see that his exit decision is described by a cutoff, $\underline{c}_\theta$, given by
\begin{equation}
  \underline{c}_\theta = \frac{1}{\xi^{1-\theta}} (\E_\mu[\tilde{\theta} \mid \omega] + \beta \Pi_\theta V_\theta),
\end{equation}
such that the seller of type $\theta$ prefers to exit if and only if $\tilde{c} > \underline{c}_\theta$.

In the case in which the seller may switch qualities, he now has two decisions to make: First, whether to exit, and second, conditional on not exiting, which quality to choose to sell. Conditional on not exiting, it is not difficult to see that the seller prefers low quality when $\tilde{c} \leq \underline{c}^*$, where
\begin{equation}
  \underline{c}^* = \frac{\beta (\Pi_1 V_1 - \Pi_0 V_0)}{1 - \xi}.
\end{equation}
Conditional on no change of the quality, a seller's exit decision is described by $\underline{c}_\theta$ as before. Hence, the seller's joint exit and quality decision is determined by $\underline{c}_\theta, \underline{c}^*$. A simplification may be made by observing that a seller who, conditional on not exiting, prefers to choose high quality, also prefers not to exit. The seller's optimal decision is summarized in the following result:
\begin{claim}
  The seller's optimal decision is described by cutoffs $\underline{c}_0, \underline{c}_1, \underline{c}^*$, such that if the seller has the option to choose a quality level, then his decision is summarized by
  \begin{equation}
    \tau(\omega, \theta, c) = \begin{cases} \text{Exit} & c > \underline{c}_0 \\ \theta = 0 & c \in [\underline{c}^*, \underline{c}^0] \\ \theta = 1 & c < \underline{c}^*.\end{cases}
  \end{equation}
\end{claim}


==> section/omitted.tex <==
%!TeX root = ../draft.tex

\propunique*

\begin{proof}

  The proof proceeds by representing equilibria as solutions to the system of equations $0 = g(x)$ on an appropriately restricted convex domain, then arguing that the Jacobian of the function $g$ is a $P$-matrix everywhere on the domain:
  \begin{definition}
    A square matrix $A$ is a \emph{$P$-matrix} means that all its principal minors are positive definite.
  \end{definition}
  It then follows from a theorem of \cite{Gale65} that any equilibrium is unique.

  To that end, represent an equilibrium by cutoff strategies and beliefs, denoted by the vectors $\langle \vec{c}, \vec{\theta}\rangle$, indexed by states and types. The equilibrium conditions are
  \begin{align}
    \vec{c}   & = (1 - \beta) p(\vec{\mu}) + \beta \Pi \bigg(\rho(\vec{c}) \big(\vec{c} - \E[\tilde{c} \mid \tilde{c} \leq \vec{c}]\big)\bigg) \label{eq:eq1} \tag{OPT} \\
    \vec{\mu} & = \rho(\vec{c}) \Pi' \vec{\mu} + \vec{\eta}, \label{eq:eq2} \tag{BEL}
  \end{align}
  where
  \begin{align*}
    \rho(\vec{c}) &:= \big(\P(\tilde{c} \leq c_{\omega_0\underline{\theta}}), \cdots, \P(\tilde{c} \leq c_{\omega_{|\Omega|-1} \overline{\theta}}\big) \\
    p(\vec{\mu}) &:= \big(\E_{\mu}[\tilde{\theta} \mid \omega_0], \cdots, \E_{\mu}[\tilde{\theta} \mid \omega_{|\Omega|-1}], \E_{\mu}[\tilde{\theta} \mid \omega_0], \cdots, \E_{\mu}[\tilde{\theta} \mid \omega_{|\Omega|-1}]\big)
  \end{align*}
  are the chances of exit conditional on type and state, and the expected type conditional on state, or the average price in that state. (Conditional on being in a state, both types receive the same price, which is why $p(\vec{\mu})$ repeats itself.)

  Define
  \begin{align}
    g_1(\vec{c}, \vec{\mu}) & := (1 - \beta) p(\vec{\mu}) + \beta \Pi \bigg(\rho(\vec{c}) \big(\vec{c} - \E[\tilde{c} \mid \tilde{c} \leq \vec{c}]\big)\bigg) - \vec{c} \\
    g_2(\vec{c}, \vec{\mu}) & := \rho(\vec{c}) \Pi' \vec{\mu} + \vec{\eta} - \vec{\mu} \label{eq:g1} \\
    g(\vec{c}, \vec{\mu}) & := \left(\begin{array}{c} g_1(\vec{c}, \vec{\mu}) \\ g_2(\vec{c}, \vec{\mu}) \end{array} \right). \label{eq:g2}
  \end{align}
  Solutions to the equilibrium conditions \ref{eq:eq1} and \eqref{eq:eq2} are equivalent to solutions to $g(\vec{c}, \vec{\mu}) = 0$.

  The next step is to find the Jacobian of $g$, $Dg$, and establish that it is a $P$-matrix. This is done by decomposing $Dg$ into the block matrices
  \begin{equation}
    Dg = \left(\begin{array}{cc} Dg_1 & \tfrac{\partial}{\partial \vec{\mu}} g_1 \\ \tfrac{\partial}{\partial \vec{c}} g_2 & Dg_2 \end{array} \right),
  \end{equation}
  arguing that $Dg_1$ and $Dg_2$ are $P$-matrices, arguing that the terms in the off-diagonal blocks $\tfrac{\partial}{\partial \vec{\mu}} g_1$ and $\tfrac{\partial}{\partial \vec{c}} g_2$ may be made arbitrarily small by taking $\beta$ large and restricting the domain of $\vec{\mu}$, and that therefore the entire Jacobian $Dg$ is a $P$-matrix on the restricted domain.

  To see that $Dg_1$ and $Dg_2$ are $P$-matrices, we use the following diagonal dominance condition:
  \begin{definition}{\citep{McKenzie60}}
    A $n\times n$ square matrix $A$ is \emph{diagonally dominant} if there exist positive weights $d_1, \ldots, d_n$ such that $d_j|a_{jj}| - \left(\sum_{i \neq j} d_i|a_{ji}|\right) > 0 \,\forall j$.
  \end{definition}
  Algebra establishes that
  \begin{align}
    Dg_1 & = \beta \Pi S - I \label{eq:dg1} \\
    Dg_2 & = R \Pi' - I. \label{eq:dg2}
  \end{align}
  where $S$ is the diagonal matrix whose diagonal entries $s_{\theta\omega, \theta\omega}$ are given by
  \begin{equation*}
    s_{\theta\omega, \theta\omega} = \rho(c_{\theta\omega})(1 - \tfrac{\partial}{\partial c_{\theta\omega}} \E[\tilde{c} \mid \tilde{c} \leq c_{\theta\omega}]) + \rho'(c_{\theta\omega})(c_{\theta\omega} - \xi(c_{\theta\omega})),
  \end{equation*}
  and $R$ is the diagonal matrix whose diagonal entries $r_{\theta\omega, \theta\omega}$ are given by $\rho(c_{\theta\omega})$.

  To see that $Dg_1$ is diagonally dominant, take weights $d_{\theta\omega}$ defined by the inverse of the diagonal elements of $S$ (positive by assumption \ref{ass:costs}):
  \begin{equation*}
    d_{\theta\omega} := s_{\theta\omega,\theta\omega}^{-1}.
  \end{equation*}
  Then we have for all $\theta\omega$
  \begin{equation*}
    \beta \left(d_{\theta\omega}(1 - \pi_{\theta\omega, \theta\omega}s_{\theta\omega}) - \left(\sum_{\theta'\omega' \neq \theta\omega} d_{\theta'\omega'}\pi_{\theta\omega, \theta'\omega'}s_{\theta'\omega'}\right)\right) \\
    = d_{\theta\omega}^{-1} - \sum_{\theta'\omega'} \pi_{\theta\omega, \theta'\omega'} > 0,
  \end{equation*}
  so that $Dg_1$ is diagonally dominant. The final inequality follows from assumption \ref{ass:costs}, which implies $d_{\theta\omega}^{-1} > 1$. A result from \cite{McKenzie60} then implies that $Dg_1$ is non-singular:
  \begin{theorem}{\citep{McKenzie60}}
    If a matrix $A$ is diagonally dominant, then it is non-singular.
    \label{thm:dominant}
  \end{theorem}
  Note further that if a square matrix $A$ is diagonally dominant, then any principal submatrix is trivially also diagonally dominant. Hence, \ref{thm:dominant} implies further that $Dg_1$ is a $P$-matrix.

  To see that $Dg_2$ is a $P$-matrix, we apply similar reasoning, but to the transpose, $Dg_2' = \Pi R$, and with weights $d_{\theta\omega} = \rho(c_{\theta\omega})^{-1}$, which as before satisfy $d_{\theta\omega} > 1$ because $\rho(c_{\theta\omega}) \in (0, 1)$ by assumption \ref{ass:costs}. If a matrix is a $P$-matrix, then its transpose is also a $P$-matrix, since the principal submatrices of the transpose of a matrix are the transpose of the principal submatrices of a matrix.

  The next step is to argue that the off-diagonal block matrices of $Dg$, $\tfrac{\partial g_1}{\partial \vec{\mu}}$ and $\tfrac{\partial g_2}{\partial \vec{c}}$ can be made to vanish. Doing so requires taking $\beta$ to be large, and the total mass of entering sellers, $|\nu|$, to be small. The latter condition is not stated as a necessary condition in the proposition, for the following reason:
  \begin{lemma}
    Let $G_\alpha$ denote games parameterized by $\langle F, \Pi, \alpha\nu \rangle$, where $\alpha$ is any positive number. Then $\langle \vec{c}, \alpha\vec{\mu} \rangle$ is an equilibrium of $G_{\alpha}$ if and only if $\langle \vec{c}, \alpha' \vec{\mu} \rangle$ is an equilibrium of $G_{\alpha'}$.
    \label{lem:scale}
  \end{lemma}
  \begin{proof}
    Let $\langle \vec{c}, \alpha \vec{\mu} \rangle$ be an equilibrium of the game $G_\alpha$. Let $g_\alpha$ denote the corresponding equilibrium conditions, $g_\alpha(\vec{c}, \alpha \vec{\mu}) = 0$. Note that $\nu$ enters only linearly into the equilibrium conditions, $\mu$ enters linearly into the stationary belief conditions \eqref{eq:eq2}, and scaling $\mu$ leaves the optimality conditions \eqref{eq:eq1} unaffected, so that multiplying through by $\alpha' / \alpha$ yields $g_{\alpha'}(\vec{c}, \alpha' \vec{\mu}) = 0$.
  \end{proof}

  An implication of lemma \ref{lem:scale} is that we can bound the mass of $\mu$ by scaling the total mass of $\eta$. If we show, e.g., global invertibility for $|\eta|$ small, then we have shown global invertibility for $|\eta|$ large. A second observation is that any solution to \eqref{eq:eq1}, \eqref{eq:eq2} must satisfy the following bounds:
  \begin{lemma}
    \label{lem:bounds}
    There exist bounds $0 < \underline{\mu}(\eta) \leq \overline{\mu}(\eta)$ such that, in any equilibrium $\langle \vec{c}, \vec{\mu} \rangle$
    \begin{equation}
      \underline{\mu}(\eta) \leq \mu_{\theta\omega} \leq \overline{\mu}(\eta),
    \end{equation}
    and
    \begin{equation}
      \lim_{|\eta| \to 0} \overline{\mu}(\eta) = 0.
      \label{eq:upperboundlimit}
    \end{equation}
  \end{lemma}
  \begin{proof}
    To prove this, we consider the two extremal cases, the first in which $c_{\theta\omega} = 1\,\forall \theta, \omega$ (thus maximizing the mass of players in each state), and one in which $c_{\theta\omega} = 0 \,\forall \theta, \omega$ (thus minimizing the mass of players in each state).

    In both cases, by assumption \ref{ass:costs}, the diagonal elements of $\rho$ are strictly bounded away from 0 and 1. Hence, by assumption \ref{ass:connected}, the matrix $\rho(\vec{c}) \Pi$ is irreducible and positive recurrent for all $\vec{c}$. So, the elements of the stationary distribution of $\rho(\vec{c}) \Pi$ are strictly positive and bounded away from 0 for all $\vec{c}$, which establishes the existence of $\underline{\mu}(\eta)$ as
    \begin{equation*}
      \underline{\mu}(\eta) = \inf_{\vec{c}} \inf_{\mu \mid \mu = \rho(\vec{c}) \Pi' \mu + \eta} \min_{\theta\omega} \mu_{\theta\omega} > 0.
    \end{equation*}
    The upper bound is derived by, e.g.,
    \begin{equation}
      \overline{\mu}(\eta) = \frac{|\Theta|\times|\Omega|\times\max_{\theta \omega} \eta_{\theta \omega}}{1 - \P(\tilde{c} \leq 1)},
      \label{eq:upperbound}
    \end{equation}
    that is, at least $\P(\tilde{c} \leq 1)$ fraction of players stay in the game, and at most $|\Theta|\times|\Omega|\times\max_{\theta \omega} \eta_{\theta \omega}$ enter, which establishes the upper bound. \eqref{eq:upperboundlimit} is an immediate consequence of \eqref{eq:upperbound}.
  \end{proof}

  A corollary of lemma \ref{lem:bounds} is the following, which will be useful later:
  \begin{corollary}
    \label{cor:bounds}
    There exists bounds $\overline{M}(\eta)$ such that
    \begin{equation}
      \frac{1}{\mu_{0\omega} + \mu_{1\omega}} \leq \overline{M}(\eta).
    \end{equation}
  \end{corollary}
  \begin{proof}
    Immediate from \ref{lem:bounds}, take
    \begin{equation*}
      \overline{M}(\eta) = \frac{1}{2\underline{\mu}}.
    \end{equation*}
  \end{proof}

  From lemma \ref{lem:bounds}, we define the domain of $g$ to be the rectangle $\mathcal{D}(\eta) = [0, 1]^{|\Theta||\Omega|} \times \mathcal{M}(\Theta \times \Omega)(\eta)$, where $\mathcal{M}(\Theta \times \Omega)(\eta)$ denotes the set of measures on $\Theta \times \Omega$ satisfying
  \begin{equation*}
    \mu_{\theta\omega} \in [\underline{\mu}(\eta), \overline{\mu}(\eta)].
  \end{equation*}
  By lemma \ref{lem:bounds} and lemma \ref{lem:scale}, if we show global invertibility of $g$ on this domain for some $\vec{\eta}$, then we will have shown uniqueness of equilibria for all uniformly scaled $\vec{\eta}$ on the full domain of measures.

  It remains only to argue that $\tfrac{\partial g_1}{\partial \vec{\mu}}$ and $\tfrac{\partial g_2}{\partial \vec{c}}$ can be made to vanish for large $\beta$ and small $|\eta|$. To that end, note that the terms of $\tfrac{\partial g_1}{\partial \vec{\mu}}$ are either zero, $(1-\beta) \mu_{\overline{\theta}\omega}/(\mu_{\overline{\theta}\omega} + \mu_{\underline{\theta}\omega})^2$, or $-(1-\beta) \mu_{\underline{\theta}\omega}/(\mu_{\overline{\theta}\omega} + \mu_{\underline{\theta}\omega})^2$. Corollary \ref{cor:bounds} implies that as $\beta \to 1$ and $|\eta| \to 0$, these terms vanish. Furthermore, the terms of $\tfrac{\partial g_2}{\partial \vec{c}}$ are either 0 or linear in $\vec{\mu}$, and hence by lemma \ref{lem:scale} vanish as $|\vec{\eta}| \to 0$.

  If
  \begin{equation*}
    \left(\begin{array}{cc} Dg_1 & 0 \\ 0 & Dg_2 \end{array} \right)
  \end{equation*}
  is a $P$-matrix, then because the inequalities are strict,
  \begin{equation*}
    \left(\begin{array}{cc} Dg_1 & \tfrac{\partial}{\partial \vec{\mu}} g_1 \\ \tfrac{\partial}{\partial \vec{c}} g_2 & Dg_2 \end{array} \right),
  \end{equation*}
  is a $P$-matrix when the off-diagonal elements are small. And because $Dg_1$ and $Dg_2$ are $P$-matrices,
  \begin{equation*}
    \left(\begin{array}{cc} Dg_1 & 0 \\ 0 & Dg_2 \end{array} \right)
  \end{equation*}
  is a $P$-matrix as well, and hence, $Dg$ is a $P$-matrix for $|\vec{\eta}|$ small and $\beta$ close to 1, so $g(x) = 0$ has a unique solution for $|\vec{\eta}|$ small and $\beta$ close to one, so it has a unique solution for $\beta$ close to 1 by lemma \ref{lem:scale}.

\end{proof}


==> section/robustness.tex <==

\subsection{Monte carlo}\label{sec:simulation}

\subsection{Model fit}\label{sec:modelfit}

